Transfer Q Star: Principled Decoding for LLM Alignment

Aligning foundation models is essential for their safe and trustworthy deployment. However, traditional fine-tuning methods are computationally intensive and require updating billions of model parameters. A promising alternative, alignment via decoding, adjusts the response distribution directly without model updates to maximize a target reward $r$, thus providing a lightweight and adaptable framework for alignment. However, principled decoding methods rely on oracle access to an optimal Q-function ($Q^*$), which is often unavailable in practice. Hence, prior SoTA methods either approximate this $Q^*$ using $Q^{\pi_{\texttt{sft}}}$ (derived from the reference $\texttt{SFT}$ model) or rely on short-term rewards, resulting in sub-optimal decoding performance. In this work, we propose Transfer $Q^*$, which implicitly estimates the optimal value function for a target reward $r$ through a baseline model $\rho_{\texttt{BL}}$ aligned with a baseline reward $\rho_{\texttt{BL}}$ (which can be different from the target reward $r$). Theoretical analyses of Transfer $Q^*$ provide a rigorous characterization of its optimality, deriving an upper bound on the sub-optimality gap and identifying a hyperparameter to control the deviation from the pre-trained reference $\texttt{SFT}$ model based on user needs. Our approach significantly reduces the sub-optimality gap observed in prior SoTA methods and demonstrates superior empirical performance across key metrics such as coherence, diversity, and quality in extensive tests on several synthetic and real datasets.

==> tables/gpt4_eval.tex <==
% \begin{table}[!h]
%     \centering
%     \caption{\textbf{GPT-4 Based Evaluation.} We prompt GPT-4 to assess and rate responses generated by different decoding strategies on the same prompt on a scale from 1 to 10, focusing on criteria such as relevance, accuracy, and insightfulness. We present the GPT-4 evaluation results measured by the percentage of win-ties of our method
%  over the alternative decoding strategies on three setups as described in Table~\ref{tab:setup_indv}: Evaluation-1 (a), Evaluation-2 (b), Evaluation-3 (c). A higher win-tie percentage indicates the efficacy of our proposed method in generating contextually relevant and accurate responses.}
%     \label{tab:gpt_4_eval}
%     \resizebox{0.71\columnwidth}{!}{%
%     \begin{tabular}{lccccc}
%     \toprule
%     & & & \multicolumn{3}{c}{\textbf{Win-Tie} (\%) $\uparrow$} \\
%     \cmidrule{4-6}
%    \textbf{Ours} & vs. & \textbf{Methods} & \textbf{Evaluation-1} & \textbf{Evaluation-2} & \textbf{Evaluation-3} \\
%     \midrule

%    \name & & ARGS-SFT & 86.67 & 72.00 & 75.34 \\
%    \name & & DPO & 70.67 & 77.34 & 70.00 \\
%    \name & & ARGS-DPO &  68.00 & 71.33 & 74.00 \\
%    \name & & $\text{CD}^{--}$ & 66.67 & 65.34 & 67.34 \\
   
   
%    \bottomrule
%     \end{tabular}%
%     }
    
% \end{table}
